Design Rule Violation Hotspot Prediction Based on Neural Network Ensembles

Design rule check is a critical step in the physical design of integrated circuits to ensure manufacturability. However, it can be done only after a time-consuming detailed routing procedure, which adds drastically to the time of design iterations. With advanced technology nodes, the outcomes of global routing and detailed routing become less correlated, which adds to the difficulty of predicting design rule violations from earlier stages. In this paper, a framework based on neural network ensembles is proposed to predict design rule violation hotspots using information from placement and global routing. A soft voting structure and a PCA-based subset selection scheme are developed on top of a baseline neural network from a recent work. Experimental results show that the proposed architecture achieves significant improvement in model performance compared to the baseline case. For half of test cases, the performance is even better than random forest, a commonly-used ensemble learning model.

==> improvements.tex <==

\section{Improvements to the Neural Network Model}
\label{sec:improvements}


\subsection{Soft Voting}
\label{subsec:soft-voting}


\subsection{Subset Selection via Principal Component Analysis}
\label{subsec:PCA}

\subsection{Smart Random PCA}
\label{subsec:smartPCA}




==> prelim.tex <==

\section{Preliminaries}
\label{sec:prelim}
Ensemble learning is a machine learning paradigm that involves multiple different learners to achieve better overall performance. Random forest \cite{random-forest} is among the most well-known ensemble learning models, where a group of decision trees are combined for better accuracy of classification. Likewise, neural network ensembles, which have been studied for decades \cite{NNE90, NNE95, NNE96, NNEzhou02}, combine a group of different neural networks for better performance of prediction.

Since a neural network usually involves a large number of parameters (mostly as weights and biases), it usually suffers from overfitting the training set, which may be cured by dropout, regularization, data augmentation, or reducing the complexity of network architecture. In this paper, we focus on reducing the network complexity in the context of neural network ensembles with a feature selection scheme based on principal component analysis (PCA) \cite{PCA}. Related works on feature selection for neural network ensembles include \cite{FS92ga, FS99opitz, FS00, FS07PCA, FS10}, which select features by using different training subsets and/or based on an objective function of the features that evaluates their fitness or contribution. Our method differs from these works in that we randomly select the features in PCA-transformed linear subspace, which does not have any objective function to evaluate (which saves the training time), and does not require different training subsets for each learner (which makes it easier to be embedded on the original neural network). We also give the network architecture that embeds all components in the proposed ensemble model, which is easy to implement in ML platforms like Tensorflow \cite{tensorflow} or higher-level packages like Keras \cite{keras}.

In a recent work \cite{DAC18}, a simple neural network with one hidden layer of 20 neurons is adopted to predict the short violations after detailed routing from placed netlists. Since \cite{DAC18} does not have more details about the architecture, we assume no dropout or regularization is applied, and we use ReLU as the activation function of the hidden layer, and the sigmoid function for the only neuron in the output layer. Formally, the activation of the $i$-th neuron in the hidden layer is given by
\begin{equation}
a_{i}^{(1)}=ReLU\left(\sum_{j=1}^r w_{ji}^{(1)}x_{j}+b_{i}^{(1)}\right),~i=1,2,\dots,20,
\label{eqn:hidden}
\end{equation}
where $r$ is the number of neurons of the input layer, $x_{j}$ is the $j$-th feature (normalized, see Section~\ref{sec:model}), and $w_{ji}^{(1)}$ and $b_{i}^{(1)}$ are weights and biases of the $i$-th neuron in the hidden layer, respectively.
The activation of the output neuron is given by
\begin{equation}
a^{(2)}=\sigma\left(\sum_{i=1}^{20} w_{i}^{(2)}a_{i}^{(1)}+b^{(2)}\right),\\
\end{equation}
where $w_{i}^{(2)}$ and $b^{(2)}$ are weights and the bias of the output neuron, respectively. In these two equations,
\begin{equation*}
ReLU(x)=\begin{cases}x, & \text{if } x > 0,\\0, & \text{otherwise}\end{cases},~\sigma(x)=\frac{1}{1+e^{-x}}
\end{equation*}
are ReLU and sigmoid functions, respectively.

In this paper, we will use this neural network as the baseline model to illustrate how neural network ensembles with our feature selection scheme can improve the model performance in the task of DRC hotspot prediction.
